Learning Cluster Representatives for Approximate Nearest Neighbor Search

Developing increasingly efficient and accurate algorithms for approximate nearest neighbor search is a paramount goal in modern information retrieval. A primary approach to addressing this question is clustering, which involves partitioning the dataset into distinct groups, with each group characterized by a representative data point. By this method, retrieving the top-k data points for a query requires identifying the most relevant clusters based on their representatives -- a routing step -- and then conducting a nearest neighbor search within these clusters only, drastically reducing the search space. The objective of this thesis is not only to provide a comprehensive explanation of clustering-based approximate nearest neighbor search but also to introduce and delve into every aspect of our novel state-of-the-art method, which originated from a natural observation: The routing function solves a ranking problem, making the function amenable to learning-to-rank. The development of this intuition and applying it to maximum inner product search has led us to demonstrate that learning cluster representatives using a simple linear function significantly boosts the accuracy of clustering-based approximate nearest neighbor search.

==> chapters/b-ack.tex <==
\chapter*{Acknowledgements}
\addcontentsline{toc}{chapter}{Acknowledgements}

I wish to express my sincere gratitude to all the wonderful people 
I have had the pleasure of meeting during my studies. Their invaluable
advice and support have been instrumental in the completion of this work.

I am thankful to my supervisor, Claudio Lucchese, who, in addition to
providing his support, has enabled me to acquire new knowledge and enrich 
my academic background.

I want to thank Franco Maria Nardini, of the ISTI CNR in Pisa, for his
collaboration. His kindness and help have enabled me to gain precious
insights in the field of Information Retrieval and beyond.

Moreover, I would like to express my deepest gratitude to my co-supervisor, 
Sebastian Bruch. I am grateful for all our conversations, for his kind soul,
his patience and professionalism. His mentorship has not only enriched my
academic experience but has also had a profound impact on my professional
development.

Finally, I am deeply grateful to my family for their unwavering support 
throughout my life. I thank my mother, who has always encouraged me to 
dream big, my father, who has helped me develop a love for mathematics, 
and my sister, who has taught me the value of perseverance, have all played 
a significant role in shaping the person I am today.

